Iterative Compression of End-to-End ASR Model using AutoML

Increasing demand for on-device Automatic Speech Recognition (ASR) systems has resulted in renewed interests in developing automatic model compression techniques. Past research have shown that AutoML-based Low Rank Factorization (LRF) technique, when applied to an end-to-end Encoder-Attention-Decoder style ASR model, can achieve a speedup of up to 3.7x, outperforming laborious manual rank-selection approaches. However, we show that current AutoML-based search techniques only work up to a certain compression level, beyond which they fail to produce compressed models with acceptable word error rates (WER). In this work, we propose an iterative AutoML-based LRF approach that achieves over 5x compression without degrading the WER, thereby advancing the state-of-the-art in ASR compression.

==> automl.tex <==
\section{AutoML based ASR compression}
\label{sec:automl}

In this section we present a brief summary of the algorithm behind AutoML-based one-shot compression. Detailed description can be found in our previous work about one-shot compression~\cite{shrinkml2019}.


%Our baseline system for iterative compression follows the same setup as presented in our previous work about one-shot compression~\cite{shrinkml2019}. We invite the reader to take a look at it for a detailed description of the algorithm behind automatic compression. The following is a short summary of what can be found in the mentioned paper.


\vspace{-0.35cm}
\paragraph*{Goal} Our goal is to find the best performing model, in terms of WER, obtained by compressing the baseline model such that the overall reduction of parameters is guaranteed to be above a certain threshold.
% Alternatively, an analogical objective could be to obtain the smallest possible model such that its accuracy is not worse than of the baseline model.
% However, since it is easier to calculate reduction of parameters rather than accuracy of a compressed model, in this paper we only discuss the first approach as it enables us to quickly reject unprofitable points, as described later. Nonetheless, we expect the findings reported in this work to still hold true for the other case as well, although it might be more time consuming to run analogical experiments.




% \begin{figure}[t!]
%   \includegraphics[width=0.8\linewidth]{iter_search.pdf}
%   \caption{Iterative compression.}
%   \label{fig:iter_compression}
% \end{figure}


\vspace{-0.35cm}
\paragraph*{Automatic compression} We use LRF as our compression method~\cite{xue_restructuring_nodate,sainath_low-rank_2013,sourav}.
% That is, for each matrix $M$ considered for compression we calculate its singular value decomposition (SVD): $M = U\Sigma V^{T}$.
% We then remove all but $k$ largest singular values from $\Sigma$, together with corresponding rows/columns from matrices $U$ and $V$, thus creating an approximation: $M \approx \hat{M} = U'\Sigma'V' = U'V^{*}$.
% We refer to $k$ as \textit{compression rank} and define its \textit{energy} as $\text{tr}(\Sigma') / \text{tr}(\Sigma)$, where $\text{tr}(A)$ is trace of matrix $A$.
That is, for each matrix $M$ considered for compression we calculate its low rank approximation ($\hat{M}$) using truncated singular value decomposition (SVD): $M = U\Sigma V \approx U'\Sigma'V' = U'V^{*} = \hat{M}$, and define its \textit{energy} as: $\text{tr}(\Sigma') / \text{tr}(\Sigma)$.
We compress each matrix independently by choosing different ranks for each one of them -- we call the set of selected ranks a \textit{compression scheme} ($s$) and define its  \textit{speedup} (equivalent to compression ratio\footnote{We sometimes interchange FLOPS with number of parameters as they are closely related in our model.}) as: 
\begingroup
\setlength\abovedisplayskip{2pt}
\setlength\belowdisplayskip{4pt}
\[\text{speedup} = \frac{\text{FLOPS of baseline}} {\text{FLOPS of compressed model}}\]
\endgroup
%Following these, our original compression problem can be reduced to the question: what is the optimal compression scheme such that its speedup is above a given threshold and WER is minimized?

We automatize the process of searching for a good compression scheme by using an algorithm based on REINFORCE~\cite{zoph_neural_2016} with two reward functions, $\mathcal{R}$ and $\mathcal{R}_{v}$, used to optimize for lower WER and smaller size respectively. The algorithm tries to find the best point from a predefined set of candidates. The set is constructed manually by specifying matrices which are subject to compression and, for each matrix independently, a set of available ranks to choose from. The search process itself does not include retraining.

%To tackle this problem, we first define a search space by selecting a subset of layers/matrices which will be subject to compression and for each defining a number of available compression levels (each level represents a different rank). In the case of our MoChA model, we identified 11 layers (consisting of total 17 matrices) which could be compressed and considered 5 different compression levels for each of them (unless specified otherwise). Because each matrix is factorized independently, this constitutes a search space of $5^{17} \approx 762\times 10^9$ possible combinations.

%We use an algorithm based on REINFORCE~\cite{zoph_neural_2016} to search for the best point among the candidates in the search space and incorporate two reward functions $\mathcal{R}$ and $\mathcal{R}_v$ to guide the search towards lower WER and smaller size respectively.
%During the search, to make the algorithm run faster, each compression scheme suggested by the algorithm for evaluation is first assessed in terms of achievable compression to check if it is above the threshold. If the scheme achieves speedup below the threshold, $\mathcal{R}_{v}$ is used as reward. Otherwise, the scheme is accepted for more costly WER evaluation and $\mathcal{R}$ is used. To make the algorithm even faster, when calculating WER we use a small subset of carefully selected utterances from \textit{dev-clean} of LibriSpeech. The selected examples are enough to produce WER values highly correlated with the ones obtained by evaluating models on the full dataset while making evaluation more than 10x faster. Details about selection process of this dataset can be found in our previous paper~\cite{shrinkml2019}.


==> result_copy.tex <==
\section{Evaluation}
\label{sec:exp}

\begin{figure}[t!]
  \includegraphics[width=0.9\linewidth]{iter_wer.pdf}
  \caption{WER for MoChA model at each step of iterative compression approach. The solid lines indicate the change in WER during each compression step, and the dotted lines show the gain in performance after retraining. The red line indicate the performance gain after retraining target compressed model.}
  \label{fig:wer}
\vspace{-4mm}
\end{figure}



\begin{table*}[t]

\centering
\begin{footnotesize}
\begin{tabular}{ l l c c c c c c c } 
\hline
\textbf{Part} & \textbf{Layer} & \textbf{Search} & \textbf{Orig. dimensions} & \textbf{Orig. FLOPS [M]} & \textbf{Rank} & \textbf{New FLOPS [M]} & \textbf{Speedup} \\ 
\hline
\hline
\multirow{6}{*}{Encoder} & LSTM 0 & \cmark & 40$\times$4096, 1024$\times$4096 & 0.16, 4.29 & Full, 105 & 0.16, 0.55 & 1x, 7.8x \\  %lstm0
 & LSTM 1 & \cmark & 1024$\times$4096, 1024$\times$4096 & 4.29, 4.29 & 72, 85  & 0.37, 0.44 & 11.4x, 9.6x \\  %lstm1
 & LSTM 2 & \cmark & 1024$\times$4096, 1024$\times$4096 & 4.29, 4.29 & 82, 63  & 0.42, 0.32 & 10.0x, 13.0x \\  %lstm2
 & LSTM 3 & \cmark & 1024$\times$4096, 1024$\times$4096 & 4.29, 4.29 & 102, 81 & 0.52, 0.41 & 8.0x, 10.1x \\  %lstm3
 & LSTM 4 & \cmark & 1024$\times$4096, 1024$\times$4096 & 4.29, 4.29 & 93, 103 & 0.48, 0.53 & 8.8x, 8.0x \\  %lstm4
 & LSTM 5 & \cmark & 1024$\times$4096, 1024$\times$4096 & 4.29, 4.29 & 80, 82  & 0.41, 0.42 & 10.2x, 10.0x \\  %lstm5
\hline
\multirow{4}{*}{Attention} &enc. ctx & \cmark & 1024$\times$1024 & 1.05 & 16 & 0.03 & 32.0x \\  %enc_ctc
 & chunk enc. ctx    & \cmark & 1024$\times$1024 & 1.05 & 24 & 0.05 & 21.3x \\  %chunck_enc_ctc
 & dec. trans.       & \cmark & 1000$\times$1024 & 1.02 & 15 & 0.03 & 33.7x \\  %s_transformed
 & chunk dec. trans. & \cmark & 1000$\times$1024 & 1.02 & 17 & 0.03 & 29.8x \\  %chunk_s_transformed
\hline
Decoder & kernel & \cmark & 2645$\times$4000 & 10.58 & 130 & 0.86 & 12.2x \\  %kernel
\hline
\multirow{3}{*}{Output} & readout & \xmark & 2645$\times$1000 & 2.64 & N/A & 2.64 & 1x \\
 & output prob. & \xmark & 500$\times$10025 & 5.01 & N/A & 5.01 & 1x \\
 & embedding    & \xmark & 10025$\times$621 & 0    & N/A & 0     & 1x \\
\hline
\hline
\multicolumn{4}{r}{\multirow{2}{*}{\textbf{Overall:}}} & \multirow{2}{*}{\textbf{63.96}} & \multirow{2}{*}{N/A} & \multirow{2}{*}{\textbf{12.73}} & \multirow{2}{*}{\textbf{5.0x}} \\
\multicolumn{4}{r}{} & & & & \\
%\cline{4-8}
\hline
\end{tabular}
\end{footnotesize}
\vspace{1mm}
\caption{Break-down of the Base--2--3--4--5x compression scheme. LSTM layers contain two matrices (for projecting input and recurrent state) hence two values are reported. Layers which do not contribute much to the running-time were omitted. However, we included the embedding layer due to its considerable size (even though it has marginal impact on run-time). %It is worth noticing that at 5x compression our model becomes mainly limited by the size of the layers which were not subject to the search, with the other parts being compressed well beyond 5x to balance them out. Also, layers related to attention turned out to be the most compressible.
}
\label{tab:breakdown}
\vspace{-8mm}
\end{table*}



\subsection{Method}
% \vspace{-0.35cm}
\paragraph*{Model Architecture.} We use an end-to-end encoder-attention-decoder ASR model~\cite{asru1,asru2,Zeyer2018ImprovedTO} with unidirectional LSTMs (unit size 1024) and monotonic chunk-wise attention (MoChA)~\cite{chiu2018monotonic} as our baseline. We identified 11 layers consisting of total 17 matrices which could be compressed and considered 5 different compression levels for each of them, which constitutes a search space of $5^{17} \approx 762\times 10^9$ possible combinations.

\vspace{-0.5cm}
\paragraph*{Model Training.} The model is trained on LibriSpeech dataset~\cite{Panayotov2015Libri} using MFCC features as input and operates on a vocabulary of 10,000 byte-pair-encoded sub-word units~\cite{Sennrich2016bpe, isck1}.
The framework used for training and evaluation of word error rate (WER) is RETURNN~\cite{zeyer2018returnnAcl} with tensorflow~\cite{tensorflow2015-whitepaper} backend. 


\vspace{-0.5cm}
\paragraph*{Baseline Compression Approach.} We use the state-of-the-art AutoML-based one-shot compression~\cite{shrinkml2019} as the baseline for evaluating the performance of our approach. 





% \begin{table}[t]
% \centering
% \begin{footnotesize}
% \begin{tabular}{ l c c } 
% % \begin{tabular}{ p{0.6\linewidth}| {0.3\linewidth} } 
% \hline
% \textbf{Trajectory} & \textbf{WER} & \textbf{GPU hours}\\ 
% \hline
% \hline
% Base-2-5x &  & \\ 
% \hline
% Base-2-3-5x &  & \\ 
% \hline
% Base-2-3-4-5x &  & \\ 
% \hline
% Base-3-4-5x &  & \\ 
% \hline
% Base-3-5x &  & \\ 
% \hline
% Base-4-5x &  & \\ 
% \hline
% \end{tabular}
% \end{footnotesize}
% \vspace{1mm}
% \caption{Different trajectories considered for iterative compression.}
% \label{table:eval}
% \vspace{-6mm}
% \end{table}

\subsection{Defining Trajectories}

To perform iterative compression, we need to define a trajectory that informs the iterative search algorithm about the intermediate speedup through which it should traverse. Since a trajectory is based on the target speedup, we performed initial experiments to explore the maximum possible compression. Based on our empirical results, we found that some layers of the model used in the experiment reach the maximum compression with the target speedup of 5x (discussed in Section~\ref{}). Therefore, to evaluate our iterative compression approach we defined a series of trajectories to obtain 5x speedup, which is 35\% improvement over the state-of-the-art AutoML-based one-shot approach~\cite{shrinkml2019}. Conclusively, we define the following trajectories:
\begin{enumerate*} [label=(\roman*)]
\item Base-2x-5x
\item Base-2x-3x-5x
\item Base-2x-3x-4x-5x
\item Base-3x-5x
\item Base-3x-4x-5x
\item Base-4x-5x. 
\end{enumerate*}
%
Note that we used the increment of speedup during each step of a trajectory as a factor of 1x, but this could be any real number as per the requirements. 


\begin{figure}[t!]
  \includegraphics[width=\linewidth]{trajectories.pdf}
  \caption{WER for MoChA model for 5x compression with different granularities of steps.}
  \label{fig:trajectories}
\vspace{-4mm}
\end{figure}


\subsection{Iterative Model Compression}

To perform iterative compression, there are two parameter required in our approach: (i) target speedup, and (ii) trajectory for iterative compression. In order to estimate the first, we continue the iterations until the model can not regain the original performance (i.e., WER close to baseline) after retraining. The speedup at which we stop the iterations (i.e., when the compressed model fails to regain the original performance) is used as the ultimate target speedup. Furthermore, to define the trajectory we increase the speedup by 1x at each iteration until we reach the target speedup.

Following the above methodology, as the first step, we compressed the model with 2x speedup by exploring different energy ranges.
Specifically, we explored the energy range between 0.3 to 0.99 and found $[0.5, 0.8]$ to be the best in finding good ranks for 2x compression of the model.
We then retrained\footnote{Through the initial experiments we found that around 50 epochs were required to recover the model performance after applying SVD while increasing speedup by 1x.} the compressed 2x model in order to regain its accuracy and used it as a base for the 3x compression search.
The processes was continued with the compression-retraining phases repeated, each time increasing the speedup by 1x, until the retrained model could no longer achieve accuracy equal or better than the baseline model.
Eventually, at step 4 in our experiment (i.e., going from 4x to 5x speedup) the model could not recover the performance after retraining, thus, we stopped compressing the model further.
We then did a final round of retraining, but this time using compressed matrices to enforce selected ranks on the model's weights.
Overall, the results show that the iterative AutoML approach could find ranks for 5.0x compression along with a 7\% relative gain in accuracy (i.e., reduced WER).
The entire process is depicted in Figure~\ref{fig:wer}, with solid and dotted lines representing search/compression and retraining steps respectively, and Table~\ref{tab:breakdown} shows a breakdown of the obtained compression scheme. We observe that at 5x compression our model becomes mainly limited by the size of the layers which were not subject to the search, with the other parts being compressed well beyond 5x (i.e., around 13x) to balance them out. Interestingly, layers related to attention turned out to be the most compressible with around 28x speedup. 

\begin{figure}[t!]
  \includegraphics[width=0.9\linewidth]{trajectories-time.pdf}
  \caption{Computation time for 5x compression on MoChA model with different granularity of step. Each color indicates the specific speedup of a step and the length represents the GPU hours consumed during search for that step.}
  \label{fig:trajectories_time}
\vspace{-4mm}
\end{figure}

%   By adapting upon this range during each step of iterative compression, the model regains the accuracy after getting compressed and retrained. In Figure~\ref{fig:wer} we show the WER of the model at each step. The solid line indicates the drop in WER during each step cause by compression, and the dotted line shows the gain from a following retraining. %In the final step, the red line indicate the performance gain after retraining compressed model.


%Figure~\ref{fig:wer}, at each step the model regains the accuracy after getting compressed and retrained. Eventually, at step 4 (i.e., going from 4x to 5x speedup) the model could not recover the performance after retraining, thus, we stop compressing the model further. As a final step, we apply SVD again and training the model with compressed matrices for 50 epochs, which helps us to  regain the WER. Overall, the results show that the iterative AutoML approach could find ranks for 5.4x compression along with a 7\% relative gain in accuracy (i.e., reduced WER). 


%\si{Fig1: I'm confused by what the edges between the stars are about? Are they a directed edge, "from here to there"?}

%\si{Fig1: Also, what's the dashed horizontal line about?}

\subsection{Impact of Step Granularity}

In our iterative search approach the granularity of steps defining a trajectory is a key parameter. We present the impact of different granularity of steps on the performance of the end model and computation time for the overall search. We performed iterative search with six possible trajectories to achieve 5x compression: 
\begin{enumerate*} [label=(\roman*)]
\item Base-2x-5x
\item Base-2x-3x-5x
\item Base-2x-3x-4x-5x
\item Base-3x-5x
\item Base-3x-4x-5x
\item Base-4x-5x 
\end{enumerate*}

As shown in Figure~\ref{fig:trajectories}, we observe that a low granularity of steps yields models with better size-accuracy. This could be due to smaller distortion of weights in each step, compared to weights distortion in higher granularity steps. At the same time, the overall compute time required to perform the compression process with fine grained steps does not increase significantly even though the number of steps performed is higher.
As shown in Figure~\ref{fig:trajectories_time}, this is due to the fact that even though the trajectories with bigger step sizes have fewer steps, searching for a bigger step size takes significantly longer compute time. 
Note that for a fair comparison between trajectories of different length, we keep the same overall retraining budget (i.e., 250 epochs) for all experiments, which is allocated proportionally to the granularity of steps. 

    


\begin{figure}[t!]
    \includegraphics[width=\linewidth]{compression.pdf}
    \includegraphics[width=\linewidth]{exynos9octa9810.pdf}
  \caption{Model compression achieved by our system (top) and measured improvement in runtime on an Exynos 9810 processor (bottom). Values reported in the legend are compression ratio and observed speedup of each part.}
  \label{fig:runtime}
\vspace{-4mm}
\end{figure}

\subsection{On-Device Measurements}
We measured running-time of both the baseline and the Base-2-3-4-5x models on a mobile phone equipped with an Exynos 9 Octa 9810 chipset to check in practice what is the achieved speedup of our model.
The models were run using a standard TFLite runtime.
%As shown in Fig.~\ref{fig:runtime}, the model was compressed differently at each part. 
As shown in Fig.~\ref{fig:runtime}, improvements in running-time (bottom) remain proportional to what we would expect from theoretical estimates (top). However, it is quite visible that the speedup achieved in practice does not match exactly the theoretical one.
We attribute that to the fact that most of the layers which were compressed became very small and therefore more sensitive to any kind of overhead present in the TFLite runtime.
However, we did not study the precise reason behind this mismatch and instead leave it for future work.

Overall, relative improvement over the baseline is 3.0x for the 5.0x reduction in FLOPS.
%We suspect that the mismatch between expected and observed speedups is caused by the parts of the network excluded from compression as they become a limiting factor while all other are heavily compressed.
Even though the observed speedup falls short to the theoretical one, our iterative compression approach still achieves significantly better results when compared to our previous model obtained with one-shot approach~\cite{shrinkml2019}.




%\subsection{Comparison between Iterative and One-shot Compression} 
\subsection{Why does Iterative outperform single-shot?}
To better understand differences between iterative and one-shot compression, we investigated if the one-shot compression approach fails to find the optimal ranks or the iterative compression along with retraining is a must to obtain higher compression.
To examine this, we explored two other strategies for achieving 5x speedup:
\begin{enumerate}[label=(\roman*)]
    \item Base--5x: search for 5x speedup using one-shot AutoML approach;
    \item Base--Iterative Ranks: apply the ranks found with our iterative approach with b-2-3-4-5 trajectory for 5x compression directly on the base model. 
\end{enumerate}
After compressing these models we retrained them with the same budget of 250 epochs. We used two retraining strategies: 
\begin{enumerate}[label=(\roman*)]
% \setlength{\itemindent}{-1em}
\setlength{\itemsep}{.5ex}
    \item Compressed: in this approach we keep the model in compressed form (i.e., keeping weight matrices as $U, V$) to constrain the training to maintain the compressed size;
    \item Cyclic: in this approach we tried to mimic the training scheme from iterative compression. At every 50 epochs, we compress the model but keep the full weight matrices (i.e., as $\hat{M}$) to allow training to recover from compression. However, in the final step we train the model in the compressed form to constrain the compressed size. Moreover, after every 50 epochs the learning rate is reset to its initial value. 
\end{enumerate}


\begin{table}[t]
\centering
\begin{tabular}{ l c } 
% \begin{tabular}{ p{0.6\linewidth}| {0.3\linewidth} } 
\hline
\textbf{Approach} & \textbf{WER (test-clean)}\\ 
\hline
\hline
Baseline & 8.32\\ 
\hline
Iterative Approach & 8.24 \\ 
\hline
Base--Iterative Ranks (Compressed) & 9.17 \\ 
\hline
Base--Iterative Ranks (Cyclic) & \textbf{8.19} \\ 
\hline
Base--5x (Compressed) & 10.25 \\ 
\hline
Base--5x (Cyclic) & 8.92 \\ 
\hline
\end{tabular}
\vspace{1mm}
\caption{Evaluation of different compression strategies.}
\label{table:eval}
\vspace{-6mm}
\end{table}


As can be seen in Table~\ref{table:eval}, the results show that our iterative approach is significantly better than \textit{Base--5x} approach, but when iterative ranks are applied to the baseline model (i.e., \textit{Base--Iterative Ranks} approach) we could obtain a compressed model with almost similar performance.
This indicates that there exists optimal compression schemes for large speedups that can be used to directly compress the baseline model without losing any accuracy.
However, our one-shot AutoML search fails to find good ranks which could be attributed to the fact that RL struggles to learn well as it encounters many more negative examples than positive ones when targeting large speedup.

Furthermore, the analysis of the two \textit{Base--Iterative Ranks} strategies tells us that aggressive compression schemes, even if known to be good, can not be simply applied to the baseline model in a one-shot manner.
Instead, a different training scheme (e.g., cyclic learning rate scheduling) has to be used to fully utilize their potential, which suggests a need for more research into training techniques for small models.




